CM2-Net: Continual Cross-Modal Mapping Network for Driver Action Recognition

Driver action recognition has significantly advanced in enhancing driver-vehicle interactions and ensuring driving safety by integrating multiple modalities, such as infrared and depth. Nevertheless, compared to RGB modality only, it is always laborious and costly to collect extensive data for all types of non-RGB modalities in car cabin environments. Therefore, previous works have suggested independently learning each non-RGB modality by fine-tuning a model pre-trained on RGB videos, but these methods are less effective in extracting informative features when faced with newly-incoming modalities due to large domain gaps. In contrast, we propose a Continual Cross-Modal Mapping Network (CM2-Net) to continually learn each newly-incoming modality with instructive prompts from the previously-learned modalities. Specifically, we have developed Accumulative Cross-modal Mapping Prompting (ACMP), to map the discriminative and informative features learned from previous modalities into the feature space of newly-incoming modalities. Then, when faced with newly-incoming modalities, these mapped features are able to provide effective prompts for which features should be extracted and prioritized. These prompts are accumulating throughout the continual learning process, thereby boosting further recognition performances. Extensive experiments conducted on the Drive&Act dataset demonstrate the performance superiority of CM2-Net on both uni- and multi-modal driver action recognition.

==> Sec/0_abstract.tex <==
\begin{abstract}
Driver action recognition is crucial for enhancing driver-vehicle interaction and ensuring driving safety.
% Recent studies showed that it can benefit from fusion of various modalities, such as infrared and depth videos.
Recent researches indicate that the integration of multiple modalities, such as infrared and depth videos, can significantly benefit the recognition.
% As there is not suitable pre-trained encode for these non-RGB modalities, previous works tend to directly fine-tune an RGB backbone on limited modality-specific data for them.
% However, this method fails to effectively extract features on these modalities as there a big modality gap between them and RGB.
Nevertheless, compared to RGB modality, it is always laborious and costly to collect extensive data for all types of non-RGB modalities in car cabin environments. 
Previous works often attempt to directly encode non-RGB data using large-scale RGB-based pre-trained models. 
However, this approach tends to be less effective in feature extraction and results in inferior action recognition, primarily due to the modality gap between these data types and RGB videos.
To address this issue, we propose a Continual Cross-Modal Mapping Network (CM$^2$-Net) to guide the training of encoder for new modality with the prompts from our well-pre-trained models. 
% Specifically, we design Accumulate Cross-modal Mapping Prompt (ACMP) strategy which can map the discriminative and informative features from pre-trained encoders to the new modal feature space.
% These mapped features is able to prompt which features should be retained in the training of new encoder.
% After training, this encoder is also capable for prompting the next encoder.
Specifically, we have developed the Accumulated Cross-modal Mapping Prompting (ACMP) strategy, which enables the mapping of discriminative and informative features from our well-pre-trained encoders to the new modality. 
These mapped features effectively prompt which features should be extracted and prioritized during the training of the new encoder.
% Thus, the prompts can be accumulated in coutinuously learning new modality.
The prompts can be accumulated during the continual learning process and further boost recognition performances.
Extensive experiments conducted on Drive\&Act dataset demonstrate the performance superiority of CM$^2$-Net on both uni- and multi-modal driver action recognition.


\end{abstract}
%
\begin{keywords}
Driver action recognition, cross-modal learning, continual learning
\end{keywords}

==> Sec/0_abstract_1.tex <==
\begin{abstract}
Driver action recognition, aiming to accurately identify drivers' behaviours, is crucial for enhancing driver-vehicle interactions and ensuring driving safety.
% Recent studies showed that it can benefit from fusion of various modalities, such as infrared and depth videos.
Recent researches in this area have shown the efficacy of integrating multiple modalities,
% that integrating multiple modalities, 
such as infrared and depth videos.
% can significantly benefit the recognition.
% As there is not suitable pre-trained encode for these non-RGB modalities, previous works tend to directly fine-tune an RGB backbone on limited modality-specific data for them.
% However, this method fails to effectively extract features on these modalities as there a big modality gap between them and RGB.
Nevertheless, compared to RGB modality, it is always laborious and costly to collect extensive data for \textit{all} types of non-RGB modalities in car cabin environments. 
Therefore, previous works propose to train each non-RGB modality separately using recognition models which pre-trained on RGB videos.
However, these approaches are less effective
in extracting informative features when faced with newly-incoming modalities 
% and results in inferior action recognition, primarily 
due to large domain gaps.
To address this issue, we propose a Continual Cross-Modal Mapping Network (CM$^2$-Net) to guide the training of newly-incoming modalities with the prompts from the previously-learned modalities. 
% Specifically, we design Accumulate Cross-modal Mapping Prompt (ACMP) strategy which can map the discriminative and informative features from pre-trained encoders to the new modal feature space.
% These mapped features is able to prompt which features should be retained in the training of new encoder.
% After training, this encoder is also capable for prompting the next encoder.
Specifically, we have developed the Accumulated Cross-modal Mapping Prompting (ACMP) strategy, to map the features learned from previous modalities into the feature space of newly-incoming modalities.
% which enables the mapping of discriminative and informative features from the previously-learned encoders to the feature space of newly-incoming modalities. 
Thus, when faced with newly-incoming modalities, these mapped features are able to provide effective prompts for what should be extracted and prioritized. 
% when learning new modalities.
% Thus, the prompts can be accumulated in coutinuously learning new modality.
And these prompts are accumulated during the continual learning process which can further boost recognition performances.
Extensive experiments conducted on Drive\&Act dataset demonstrate the performance superiority of CM$^2$-Net on both uni- and multi-modal driver action recognition.


\end{abstract}
%
\begin{keywords}
Driver action recognition, cross-modal learning, continual learning
\end{keywords}

==> Sec/0_abstract_2.tex <==
\begin{abstract}
Driver action recognition is crucial for enhancing driver-vehicle interactions and ensuring driving safety.
Recent research in this area has shown the efficacy of integrating multiple modalities, such as infrared and depth.
% Recent studies showed that it can benefit from fusion of various modalities, such as infrared and depth videos.
% that integrating multiple modalities, 
% can significantly benefit the recognition.
% As there is not suitable pre-trained encode for these non-RGB modalities, previous works tend to directly fine-tune an RGB backbone on limited modality-specific data for them.
% However, this method fails to effectively extract features on these modalities as there a big modality gap between them and RGB.
Nevertheless, compared to RGB modality, it is always laborious and costly to collect extensive data for all types of non-RGB modalities in car cabin environments. 
Previous works suggest independently learning each non-RGB modality by fine-tuning a model pre-trained on RGB videos, but these methods struggle to extract informative features when faced with newly-incoming modalities due to large domain gaps.
On the contrary, we propose a Continual Cross-Modal Mapping Network (CM$^2$-Net) to guide the learning of each newly-incoming modality with prompts from the previously-learned modalities. 
% Specifically, we design Accumulate Cross-modal Mapping Prompt (ACMP) strategy which can map the discriminative and informative features from pre-trained encoders to the new modal feature space.
% These mapped features is able to prompt which features should be retained in the training of new encoder.
% After training, this encoder is also capable for prompting the next encoder.
Specifically, we have developed Accumulative Cross-modal Mapping Prompting (ACMP), to map the discriminative and informative features learned from previous modalities into the feature space of newly-incoming modalities.
Then, when faced with newly-incoming modalities, these mapped features are able to provide effective prompts for which features should be extracted and prioritized. 
These prompts are accumulating throughout the continual learning process, thereby boosting further recognition performances.
Extensive experiments conducted on the Drive\&Act dataset demonstrate the performance superiority of CM$^2$-Net on both uni- and multi-modal driver action recognition.
% which enables the mapping of discriminative and informative features from the previously-learned encoders to the feature space of newly-incoming modalities. 
% when learning new modalities.
% Thus, the prompts can be accumulated in coutinuously learning new modality.


\end{abstract}
%
\begin{keywords}
Driver action recognition, cross-modal learning, continual learning
\end{keywords}

==> Sec/0_abstract_legacy.tex <==
\begin{abstract}
Driver action recognition is crucial for enhancing driver-vehicle interaction and ensuring driving safety.
% Recent studies showed that it can benefit from fusion of various modalities, such as infrared and depth videos.
Recent research indicates that the integration of multiple modalities, 
such as infrared and depth videos.
can significantly benefit the recognition.
% As there is not suitable pre-trained encode for these non-RGB modalities, previous works tend to directly fine-tune an RGB backbone on limited modality-specific data for them.
% However, this method fails to effectively extract features on these modalities as there a big modality gap between them and RGB.
Previous works 
often attempt to directly encode non-RGB data using large-scale RGB-based 
pre-trained 
models. 
However, this approach tends to be less effective in feature extraction and results in inferior action recognition, primarily due to the modality gap between these data types and RGB videos.
To address this issue, we propose a Continual Cross-Modal Mapping Network (CM$^2$-Net) to guide the training of encoder for new modality with the prompts from our well-pre-trained models. 
% Specifically, we design Accumulate Cross-modal Mapping Prompt (ACMP) strategy which can map the discriminative and informative features from pre-trained encoders to the new modal feature space.
% These mapped features is able to prompt which features should be retained in the training of new encoder.
% After training, this encoder is also capable for prompting the next encoder.
Specifically, we have developed the Accumulated Cross-modal Mapping Prompting (ACMP) strategy, which enables the mapping of discriminative and informative features from our well-pre-trained encoders to the new modality. 
These mapped features effectively prompt which features should be extracted and prioritized during the training of the new encoder.
% Thus, the prompts can be accumulated in coutinuously learning new modality.
The prompts can be accumulated in continually learning new modalities.
Extensive experiments conducted on Drive\&Act dataset demonstrate the performance superiority of CM$^2$-Net on both uni- and multi-modal driver action recognition.


\end{abstract}
%
\begin{keywords}
Driver action recognition, cross-modal learning, continual learning
\end{keywords}

==> tabs/ablation1.tex <==
\begin{table}[htbp]
\caption{The comparison with the existing methods pre-trained on multi-modal dataset using same backbone UniFormerV2.}
\begin{center}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lccc}
\hline
Training &  Modality & Top-1 & Mean-1 \\ 
\hline
Pretrained on NTU RGB+D~\cite{nturgbd}  & Depth & 69.21 & 56.35\\ 
\textbf{ACMG} & Depth & \textbf{76.40} & \textbf{60.17} \\
\hline
Pretrained on NTU RGB+D~\cite{nturgbd} & IR & 72.56 & 59.64\\ 
\textbf{ACMG} & IR & \textbf{80.27} & \textbf{64.02} \\
\hline
Pretrained on K710~\cite{uniformerv2} & RGB & 81.99 & 67.79\\ 
\textbf{ACMG} & RGB & \textbf{83.51} & \textbf{69.76} \\
\hline
\end{tabular}
}
\label{Ablation study 1}
\end{center}
\end{table}

==> tabs/ablation2.tex <==
\begin{table}[htbp]
\caption{The comparison with existing methods adopting RGB encoder using the same backbone UniFormerV2.}
\begin{center}
\begin{tabular}{lccc}
\hline
Training &  Modality & Top-1 & Mean-1 \\ 
\hline
Adopt RGB encoder  & Depth & 69.21 & 56.35\\ 
\textbf{ACMG} & Depth & \textbf{76.40} & \textbf{60.17} \\
\hline
Adopt RGB encoder & IR & 72.56 & 59.64\\ 
\textbf{ACMG} & IR & \textbf{80.27} & \textbf{64.02} \\
\hline
\end{tabular}
\label{Ablation study 2}
\end{center}
\end{table}

==> tabs/ablation_studu.tex <==
\begin{table}[htbp]
\caption{Ablation study on the impact of ACMG prompting modalities.}
\begin{center}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{cclcc}
\hline
Method & Modality & Prompt & Top-1 & Mean-1 \\
\hline
\multirow{5}{*}{\textbf{CM$^2$-Net}} & \multirow{2}{*}{\textbf{IR}} & \textbf{w/} RGB & \textbf{80.46} & \textbf{64.97} \\
& & \textbf{w/o} RGB & 79.36 & 62.56 \\
\cline{2-5}
& \multirow{3}{*}{\textbf{Depth}} & \textbf{w/} RGB \& IR & \textbf{76.48} & \textbf{63.01} \\
& & \textbf{w/} RGB  & 76.30 & 62.28 \\
& & \textbf{w/o} RGB/IR  & 73.89 & 54.85 \\
\hline
\end{tabular}
\label{Ablation study 0}
}
\end{center}
\end{table}
